Visually Dehallucinative Instruction Generation

In recent years, synthetic visual instructions by generative language model have demonstrated plausible text generation performance on the visual question-answering tasks. However, challenges persist in the hallucination of generative language models, i.e., the generated image-text data contains unintended contents. This paper presents a novel and scalable method for generating visually dehallucinative instructions, dubbed CAP2QA, that constrains the scope to only image contents. Our key contributions lie in introducing image-aligned instructive QA dataset CAP2QA-COCO and its scalable recipe. In our experiments, we compare synthetic visual instruction datasets that share the same source data by visual instruction tuning and conduct general visual recognition tasks. It shows that our proposed method significantly reduces visual hallucination while consistently improving visual recognition ability and expressiveness.

==> figure_template <==
\begin{figure}[htb]

\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=8.5cm]{image1}}
%  \vspace{2.0cm}
  \centerline{(a) Result 1}\medskip
\end{minipage}
%
\begin{minipage}[b]{.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image3}}
%  \vspace{1.5cm}
  \centerline{(b) Results 3}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image4}}
%  \vspace{1.5cm}
  \centerline{(c) Result 4}\medskip
\end{minipage}
%
\caption{Example of placing a figure with experimental results.}
\label{fig:res}
%
\end{figure}


==> fs/figure_metrics.tex <==
\begin{figure}[!h]
\centering
%\begin{minipage}[]{0.7\linewidth}
%  \centering
%  \centerline{\includegraphics[width=1.0\linewidth]{fs/metrics_pic.png}}
%  \centerline{}\medskip
%\end{minipage}
%\vspace{-2em}

\begin{minipage}[]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=1.0\linewidth]{fs/metric_v3.png}}
\end{minipage}

\caption{
PAcc enables evaluating sentences on the existing data with flexibility in inflections.
}
\label{fig:metrics}

\end{figure}

==> fs/table_metrics.tex <==
\begin{table}[h]
\centering
\caption{metrics}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c}
\toprule
\multicolumn{3}{c}{GTs: ['sail', 'sail', 'sail', 'sail', 'sail', 'sail', 'travel', 'travel', 'fish', 'fish']} \\ 
Answer & Acc & PAcc \\ \hline
sail & 1.0 & 1.0 \\
fish & 0.67 & 0.67 \\
sailing & 0 & 1.0 \\
fishing & 0 & 0.67 \\
They are used for fishing & 0 & 1.0 \\
\bottomrule
\end{tabular}
}
\label{table:metrics}
\end{table}

